GraPhSyM: Graph Physical Synthesis Model

In this work, we introduce GraPhSyM, a Graph Attention Network (GATv2) model for fast and accurate estimation of post-physical synthesis circuit delay and area metrics from pre-physical synthesis circuit netlists. Once trained, GraPhSyM provides accurate visibility of final design metrics to early EDA stages, such as logic synthesis, without running the slow physical synthesis flow, enabling global co-optimization across stages. Additionally, the swift and precise feedback provided by GraPhSyM is instrumental for machine-learning-based EDA optimization frameworks. Given a gate-level netlist of a circuit represented as a graph, GraPhSyM utilizes graph structure, connectivity, and electrical property features to predict the impact of physical synthesis transformations such as buffer insertion and gate sizing. When trained on a dataset of 6000 prefix adder designs synthesized at an aggressive delay target, GraPhSyM can accurately predict the post-synthesis delay (98.3%) and area (96.1%) metrics of unseen adders with a fast 0.22s inference time. Furthermore, we illustrate the compositionality of GraPhSyM by employing the model trained on a fixed delay target to accurately anticipate post-synthesis metrics at a variety of unseen delay targets. Lastly, we report promising generalization capabilities of the GraPhSyM model when it is evaluated on circuits different from the adders it was exclusively trained on. The results show the potential for GraPhSyM to serve as a powerful tool for advanced optimization techniques and as an oracle for EDA machine learning frameworks.

==> algo_ppg.tex <==

\begin{algorithm}[htbp]
\scriptsize

\SetAlgoLined
% Set Function Names
\SetKwFunction{FInit}{Initialize}
\SetKwFunction{FAdd}{Add}
\SetKwFunction{FDel}{Delete}
\SetKwFunction{FLeg}{Legalize}

\SetKwProg{Fn}{Function}{:}{}
\Fn{\FInit}{
 $nodelist \leftarrow \emptyset, minlist \leftarrow \emptyset$\;
 \For(\tcp*[f]{add in/out nodes}){$m\leftarrow 0$ \KwTo $(N-1)$}{
  add $(m,m)$, $(m,0)$ to $nodelist$
 }
}

\SetKwProg{Fn}{Function}{:}{}
\Fn{\FAdd{msb,lsb}}{
 add $(msb,lsb)$ to $minlist$\;
 \tcp{remove new node's and child's lps from minlist}
 \For{$l\leftarrow (msb-1)$ \KwTo $0$}{
  \If{$(msb,l)$ is in $minlist$}{
   delete $lp(msb,l)$ from $minlist$
  }
 }
 \FLeg{}
}

\SetKwProg{Fn}{Function}{:}{}
\Fn{\FDel{msb,lsb}}{
 delete $(msb,lsb)$ from $minlist$\;
 \FLeg{}
}
\SetKwProg{Fn}{Function}{:}{}
\Fn{\FLeg}{
 $nodelist \longleftarrow minlist$\;
 \For(\tcp*[f]{add in/out nodes}){$m\leftarrow 0$ \KwTo $(N-1)$}{
  add $(m,m)$, $(m,0)$ to $nodelist$
 }
 \For(\tcp*[f]{add missing lps}){$m\leftarrow (N-1)$ \KwTo $0$}{
  \For{$l\leftarrow (m-1)$ \KwTo $0$}{
   \If{$(m,l)$ is in $nodelist$}{
    add $lp(m,l)$ to $nodelist$
   }
  }
 }
}

\caption{\small PrefixRL N-input prefix graph actions}
\label{algo:pgg}
\end{algorithm}

==> figtex/fig_analyticalresults.tex <==
\begin{figure}[htbp]
    %\setlength{\abovecaptionskip}{3pt}
    \setlength{\belowcaptionskip}{0pt}
    \centering
    \begin{subfigure}[b]{0.5\linewidth}
        \setlength{\abovecaptionskip}{0pt}
        \setlength{\belowcaptionskip}{0pt}
        \centering
        \includegraphics[width=\textwidth]{figs/fig_32b_analytical_pure.pdf}
         \caption{Analytical Metrics.}
        \label{fig:32anaresultsana}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[b]{0.5\linewidth}
        \setlength{\abovecaptionskip}{0pt}
        \setlength{\belowcaptionskip}{0pt}
        \centering
        \includegraphics[width=\textwidth]{figs/fig_32b_analytical_synth.pdf}
        \caption{Synthesized Metrics.}
        \label{fig:32anaresultssynth}
    \end{subfigure}%
        \caption{32b Analytical-PrefixRL adders outperform SA\cite{moto2018prefix} and PS\cite{roy2014towards} adders when trained and compared with analytical metrics from \cite{moto2018prefix}. However, timing-driven synthesis optimizations in OpenPhySyn optimize the PS adders better than the Analytical-PrefixRL and SA adders in synthesized circuits. PrefixRL adders trained with OpenPhySyn synthesis in-the-loop have the best performing synthesized circuits.}
        \label{fig:32anaresults}
\end{figure}

==> figtex/fig_commercialresults.tex <==
\begin{figure}
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\belowcaptionskip}{-10pt}
    \centering
    \begin{subfigure}[b]{\linewidth}
        \setlength{\abovecaptionskip}{0pt}
        \setlength{\belowcaptionskip}{0pt}
        \centering
        \includegraphics[width=\textwidth]{figs/fig_32b_commercial.pdf}
        \caption{32b Adder Synthesis. Commercial tool, 8nm.}
        \label{fig:commercialresults32}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[b]{\linewidth}
        \setlength{\abovecaptionskip}{0pt}
        \setlength{\belowcaptionskip}{0pt}
        \centering
        \includegraphics[width=\textwidth]{figs/fig_64b_commercial.pdf}
        \caption{64b Adder Synthesis. Commercial tool, 8nm.}
        \label{fig:commercialresults64}
    \end{subfigure}%
        \caption{Area-delay Pareto curves for 32b and 64b adders synthesized using a Commercial Synthesis Tool. Despite having been trained only with OpenPhySyn, PrefixRL-generated adders still Pareto-dominate existing baselines at all but the lowest delay target.
        (Sklansky\cite{sklansky1960conditional}, KoggeStone\cite{kogge1973a}, BrentKung\cite{brent1982a})}
        \label{fig:commercialresults}
\end{figure}

==> figtex/fig_openphysynresults.tex <==
\begin{figure}
    \setlength{\abovecaptionskip}{3pt}
    \setlength{\belowcaptionskip}{-10pt}
    \centering
    \begin{subfigure}[b]{\linewidth}
        \setlength{\abovecaptionskip}{0pt}
        \setlength{\belowcaptionskip}{0pt}
        \centering
        \includegraphics[width=\textwidth]{figs/fig_32b_openphysyn.pdf}
        \caption{32b Adder Synthesis. OpenPhySyn, Nangate45.}
        \label{fig:openphysynresults32}
    \end{subfigure}%
    \hfill%
    \begin{subfigure}[b]{\linewidth}
        \setlength{\abovecaptionskip}{0pt}
        \setlength{\belowcaptionskip}{0pt}
        \centering
        \includegraphics[width=\textwidth]{figs/fig_64b_openphysyn.pdf}
        \caption{64b Adder Synthesis. OpenPhySyn, Nangate45.}
        \label{fig:openphysynresults64}
    \end{subfigure}%
        \caption{Area-delay Pareto curves for 32b and 64b adders synthesized with OpenPhySyn. PrefixRL adders Pareto-dominate all prior work.
        (Sklansky\cite{sklansky1960conditional}, KoggeStone\cite{kogge1973a}, BrentKung\cite{brent1982a}, SA\cite{moto2018prefix}, PS\cite{roy2014towards}, CL\cite{ma2019cross})
        }
        \label{fig:openphysynresults}
\end{figure}

==> figtex/fig_scaling.tex <==
\begin{table}[htbp]
  \centering
  \caption{Comparison of 16b, 32b and 64b PrefixRL adder design}
    \resizebox{\columnwidth}{!}{\begin{tabular}{cccc}
    \textbf{Statistic} & \multicolumn{1}{M{5.145em}}{\textbf{16b}} & \multicolumn{1}{M{5em}}{\textbf{32b}} & \multicolumn{1}{M{5.785em}}{\textbf{64b}} \\
    \toprule
    \textbf{$\vert \mathcal{A} \vert$} & 105 & 465 & 1953 \\
    \textbf{Synthesis time} & 11.39s & 16.85s & 35.56s \\ 
    \textbf{Train iteration time} & 0.45s & 1.61s & 3.15s \\
    \textbf{\# of residual blocks} & 16 & 32 & 32 \\
    \textbf{per-GPU batch size} & 96 & 96 & 6 \\
    \textbf{\# of data-parallel GPUs} & 1 & 1 & 14 \\
    \bottomrule
    \end{tabular}}%
\begin{tablenotes}[flushleft]
\item 
Synthesis times are for Sklansky adders evaluated at 4 timing constraints. The problem space grows quickly with the number of bits and impacts other details of training.  
\end{tablenotes}
  \label{fig-scaling}%
\end{table}%


==> results.tex <==
% Table generated by Excel2LaTeX from sheet 'table'
\begin{table}[htbp]
  \centering
  \caption{Experimental results For 32B Adder Optimization}\label{tab:results}
    \begin{tabular}{c|cc|cc|c|cc}
    \hline
    Design & \multicolumn{2}{c|}{Analytical} & \multicolumn{2}{c|}{Physical} & w\textsubscript{delay} & \multicolumn{2}{c}{Steps} \\
\cline{2-5}\cline{7-8}        & Area & Delay & Area & Delay &     & Gen. & Learn \\
    \hline
    RL01 & 53 & 20.0 & 1.000 & 1.448 & 0.08 & 13  & 1.45M \\
    RL02 & 54 & 18.0 & 1.010 & 1.307 & 0.12 & 15  & 2.05M \\
    RL03 & 55 & 17.5 & 1.020 & 1.223 & 0.10 & 16  & 1.46M \\
    RL04 & 56 & 17.0 & 1.030 & 1.193 & 0.15 & 15  & 1.42M \\
    RL05 & 57 & 16.5 & 1.040 & 1.185 & 0.20 & 18  & 1.34M \\
    RL06 & 59 & 16.0 & 1.060 & 1.153 & 0.25 & 18  & 3.41M \\
    RL07 & 60 & 15.5 & 1.069 & 1.153 & 0.25 & 18  & 2.63M \\
    RL08 & 63 & 15.0 & 1.099 & 1.107 & 0.45 & 13  & 2.39M \\
    RL09 & 66 & 14.5 & 1.129 & 1.078 & 0.50 & 19  & 2.69M \\
    RL10 & 70 & 14.0 & 1.169 & 1.053 & 0.70 & 20  & 2.32M \\
    RL11 & 76 & 13.5 & 1.228 & 1.000 & 0.70 & 26  & 3.56M \\
    RL12 & 83 & 13.0 & 1.298 & 1.006 & 0.95 & 30  & 3.02M \\
    \hline
    SA01 & 53 & 20.5 & 1.000 & 1.460 & -   & -   & - \\
    SA02 & 54 & 18.5 & 1.010 & 1.368 & -   & -   & - \\
    SA03 & 57 & 17.0 & 1.040 & 1.221 & -   & -   & - \\
    SA04 & 65 & 15.5 & 1.119 & 1.126 & -   & -   & - \\
    SA05 & 73 & 14.5 & 1.199 & 1.099 & -   & -   & - \\
    SA06 & 94 & 13.0 & 1.407 & 1.002 & -   & -   & - \\
    \hline
    ES01 & 74 & 21.0 & 1.208 & 1.271 & -   & -   & - \\
    ES02 & 56 & 19.5 & 1.030 & 1.371 & -   & -   & - \\
    \hline
    Sklansky & 80  & 23.5 & 1.268 & 1.395 & -   & -   & - \\
    KoggeStone & 129 & 15.5 & 1.754 & 1.048 & -   & -   & - \\
    BrentKung & 57  & 23.0 & 1.040 & 1.578 & -   & -   & - \\
    \hline
    \hline
\multicolumn{8}{l}{RL* designs are generates from PrefixRL agents}\\
\multicolumn{8}{l}{ES* designs are obtained from Exhaustive Search (ES) with pruning\cite{roy2014towards}}\\
\multicolumn{8}{l}{SA* designs are obtained from Simulated Annealing (SA)\cite{moto2018prefix}}\\
\multicolumn{8}{l}{Sklanksy, KoggeStone and BrentKung are regular structures \cite{sklansky1960conditional, kogge1973a, brent1982a}}\\
\multicolumn{8}{l}{Physical metrics are normalized}\\
\multicolumn{8}{l}{Scalarization weight w\textsubscript{area}$ = 1-$w\textsubscript{delay}}\\
\end{tabular}%
  \label{tab:addlabel}%
\end{table}%


==> results_analytical.tex <==
% Table generated by Excel2LaTeX from sheet 'table'
\begin{table}[htbp]
  \centering
  \caption{Analytical metrics for 32b Adder Optimization}\label{tab:results_analytical}
    \begin{tabular}{c|cc|c|cc}
    \hline
    Design & Area & Delay & w\textsubscript{delay} & \multicolumn{2}{c}{Steps} \\
\cline{5-6}        &  &  &     & Gen. & Learn \\
    \hline
    RL01 & 53 & 20.0 & 0.08 & 13  & 1.45M \\
    RL02 & 54 & 18.0 & 0.12 & 15  & 2.05M \\
    RL03 & 55 & 17.5 & 0.10 & 16  & 1.46M \\
    RL04 & 56 & 17.0 & 0.15 & 15  & 1.42M \\
    RL05 & 57 & 16.5 & 0.20 & 18  & 1.34M \\
    RL06 & 59 & 16.0 & 0.25 & 18  & 3.41M \\
    RL07 & 60 & 15.5 & 0.25 & 18  & 2.63M \\
    RL08 & 63 & 15.0 & 0.45 & 13  & 2.39M \\
    RL09 & 66 & 14.5 & 0.50 & 19  & 2.69M \\
    RL10 & 70 & 14.0 & 0.70 & 20  & 2.32M \\
    RL11 & 76 & 13.5 & 0.70 & 26  & 3.56M \\
    RL12 & 83 & 13.0 & 0.95 & 30  & 3.02M \\
    \hline
    SA01 & 53 & 20.5 & -   & -   & - \\
    SA02 & 54 & 18.5 & -   & -   & - \\
    SA03 & 57 & 17.0 & -   & -   & - \\
    SA04 & 65 & 15.5 & -   & -   & - \\
    SA05 & 73 & 14.5 & -   & -   & - \\
    SA06 & 94 & 13.0 & -   & -   & - \\
    \hline
    ES01 & 74 & 21.0 & -   & -   & - \\
    ES02 & 56 & 19.5 & -   & -   & - \\
    \hline
    Sklansky \cite{sklansky1960conditional} & 80  & 23.5 & -   & -   & - \\
    KoggeStone \cite{kogge1973a} & 129 & 15.5 & -   & -   & - \\
    BrentKung \cite{brent1982a} & 57  & 23.0 & -   & -   & - \\
    \hline
    \hline
\multicolumn{6}{l}{RL*: Generated from PrefixRL agents}\\
\multicolumn{6}{l}{ES*: Exhaustive Search (ES) with pruning\cite{roy2014towards}}\\
\multicolumn{6}{l}{SA*: Simulated Annealing (SA)\cite{moto2018prefix}}\\
\multicolumn{6}{l}{Scalarization weight w\textsubscript{area}$ = 1-$w\textsubscript{delay}}\\
\end{tabular}%
  \label{tab:addlabel}%
\end{table}%


==> results_synthesized.tex <==
% Table generated by Excel2LaTeX from sheet 'table'
\begin{table}[htbp]
  \centering
  \caption{Synthesized metrics for 32B Adder Optimization}\label{tab:results_synthesized}
    \begin{tabular}{c|cc}
    \hline
    Design & Area & Delay \\
    \hline
    RL01 & 1.000 & 1.448 \\
    RL02 & 1.010 & 1.307 \\
    RL03 & 1.020 & 1.223 \\
    RL04 & 1.030 & 1.193 \\
    RL05 & 1.040 & 1.185 \\
    RL06 & 1.060 & 1.153 \\
    RL07 & 1.069 & 1.153 \\
    RL08 & 1.099 & 1.107 \\
    RL09 & 1.129 & 1.078 \\
    RL10 & 1.169 & 1.053 \\
    RL11 & 1.228 & 1.000 \\
    RL12 & 1.298 & 1.006 \\
    \hline
    SA01 & 1.000 & 1.460 \\
    SA02 & 1.010 & 1.368 \\
    SA03 & 1.040 & 1.221 \\
    SA04 & 1.119 & 1.126 \\
    SA05 & 1.199 & 1.099 \\
    SA06 & 1.407 & 1.002 \\
    \hline
    ES01 & 1.208 & 1.271 \\
    ES02 & 1.030 & 1.371 \\
    \hline
    Sklansky \cite{sklansky1960conditional} & 1.268 & 1.395 \\
    KoggeStone \cite{kogge1973a} & 1.754 & 1.048 \\
    BrentKung \cite{brent1982a} & 1.040 & 1.578 \\
    \hline
    \hline
\multicolumn{3}{l}{RL*: Generated from PrefixRL agents}\\
\multicolumn{3}{l}{ES*: Exhaustive Search (ES) with pruning\cite{roy2014towards}}\\
\multicolumn{3}{l}{SA*: Simulated Annealing (SA)\cite{moto2018prefix}}\\
\multicolumn{3}{l}{Synthesized area and delay metrics are normalized\textsuperscript{\ref{fn:technode}}}\\

\end{tabular}%
  \label{tab:addlabel}%
\end{table}%

